Plausible presence of new state in neutron stars with masses above $0.98M_{\rm TOV}$

We investigate the neutron star (NS) equation of state (EOS) by incorporating multi-messenger data of GW170817, PSR J0030+0451, PSR J0740+6620, and state-of-the-art theoretical progresses, including the information from chiral effective field theory ($\chi$EFT) and perturbative quantum chromodynamics (pQCD) calculation. Taking advantage of the various structures sampling by a single-layer feed-forward neural network model embedded in the Bayesian nonparametric inference, the structure of NS matter's sound speed $c_{\rm s}$ is explored in a model-agnostic way. It is found that a peak structure is common in the $c_{\rm s}^2$ posterior, locating at $2.4-4.8\rho_{\rm sat}$ (nuclear saturation density) and $c_{\rm s}^2$ exceeds ${c^{2}}/{3}$ at 90\% credibility. The non-monotonic behavior suggests evidence of the state deviating from hadronic matter inside the very massive NSs. Assuming the new/exotic state is featured as it is softer than typical hadronic models or even with hyperons, we find that a sizable ($\geq 10^{-3}M_\odot$) exotic core, likely made of quark matter, is plausible for the NS with a gravitational mass above about $0.98M_{\rm TOV}$, where $M_{\rm TOV}$ represents the maximum gravitational mass of a non-rotating cold NS. The inferred $M_{\rm TOV} = 2.18^{+0.27}_{-0.13}M_\odot$ (90\% credibility) is well consistent with the value of $2.17^{+0.15}_{-0.12}M_\odot$ estimated independently with GW170817/GRB 170817A/AT2017gfo assuming a temporary supramassive NS remnant formed after the merger. PSR J0740+6620, the most massive NS detected so far, may host an exotic core with a probability of $\approx 0.36$.

==> aas_macros.tex <==
%
%  These Macros are taken from the AAS TeX macro package version 5.2
%  and are compatible with the macros in the A&A document class
%  version 7.0
%  Include this file in your LaTeX source only if you are not using
%  the AAS TeX macro package or the A&A document class and need to
%  resolve the macro definitions in the TeX/BibTeX entries returned by
%  the ADS abstract service.
%
%  If you plan not to use this file to resolve the journal macros
%  rather than the whole AAS TeX macro package, you should save the
%  file as ``aas_macros.sty'' and then include it in your LaTeX paper
%  by using a construct such as:
% \documentstyle[11pt,aas_macros]{article~~}
%
%  For more information on the AASTeX and A&A packages, please see:
%       http://journals.aas.org/authors/aastex.html 
%       ftp://ftp.edpsciences.org/pub/aa/readme.html
%  For more information about ADS abstract server, please see:
%       http://adsabs.harvard.edu/ads_abstracts.html
%

% Abbreviations for journals.  The object here is to provide authors
% with convenient shorthands for the most "popular" (often-cited)
% journals; the author can use these markup tags without being concerned
% about the exact form of the journal abbreviation, or its formatting.
% It is up to the keeper of the macros to make sure the macros expand
% to the proper text.  If macro package writers agree to all use the
% same TeX command name, authors only have to remember one thing, and
% the style file will take care of editorial preferences.  This also
% applies when a single journal decides to revamp its abbreviating
% scheme, as happened with the ApJ (Abt 1991).

\def\aj{AJ~}                   % Astronomical Journal
\def\actaa{Acta Astron~}      % Acta Astronomica
\def\araa{ARA\&A~}             % Annual Review of Astron and Astrophys
\def\apj{ApJ~}                 % Astrophysical Journal
\def\apjl{ApJL~}                % Astrophysical Journal, Letters
\def\apjs{ApJS~}               % Astrophysical Journal, Supplement
\def\ao{Appl~Opt~}           % Applied Optics
\def\apss{Ap\&SS~}             % Astrophysics and Space Science
\def\aap{A\&A~}                % Astronomy and Astrophysics
\def\aapr{A\&A~Rev~}          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS~}              % Astronomy and Astrophysics, Supplement
\def\azh{AZh~}                 % Astronomicheskii Zhurnal
\def\baas{BAAS~}               % Bulletin of the AAS
\def\bac{Bull astr Inst Czechosl~}
                % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{Chinese Astron Astrophys~}
                % Chinese Astronomy and Astrophysics
\def\cjaa{Chinese J Astron Astrophys~}
                % Chinese Journal of Astronomy and Astrophysics
\def\icarus{Icarus~}           % Icarus
\def\jcap{J Cosmology Astropart Phys~}
                % Journal of Cosmology and Astroparticle Physics
\def\jrasc{JRASC~}             % Journal of the RAS of Canada
\def\memras{MmRAS~}            % Memoirs of the RAS
\def\mnras{MNRAS~}             % Monthly Notices of the RAS
\def\na{New A~}                % New Astronomy
\def\nar{New A Rev~}          % New Astronomy Review
\def\pra{Phys~Rev~A~}        % Physical Review A: General Physics
\def\prb{Phys~Rev~B~}        % Physical Review B: Solid State
\def\prc{Phys~Rev~C~}        % Physical Review C
\def\prd{Phys~Rev~D~}        % Physical Review D
\def\pre{Phys~Rev~E~}        % Physical Review E
\def\prl{Phys~Rev~Lett~}    % Physical Review Letters
\def\pasa{PASA~}               % Publications of the Astron. Soc. of Australia
\def\pasp{PASP~}               % Publications of the ASP
\def\pasj{PASJ~}               % Publications of the ASJ
\def\rmxaa{Rev Mexicana Astron Astrofis~}%
                % Revista Mexicana de Astronomia y Astrofisica
\def\qjras{QJRAS~}             % Quarterly Journal of the RAS
\def\skytel{S\&T~}             % Sky and Telescope
\def\solphys{Sol~Phys~}      % Solar Physics
\def\sovast{Soviet~Ast~}      % Soviet Astronomy
\def\ssr{Space~Sci~Rev~}     % Space Science Reviews
\def\zap{ZAp~}                 % Zeitschrift fuer Astrophysik
\def\nat{Nature~}              % Nature
\def\iaucirc{IAU~Circ~}       % IAU Cirulars
\def\aplett{Astrophys~Lett~} % Astrophysics Letters
\def\apspr{Astrophys~Space~Phys~Res~}
                % Astrophysics Space Physics Research
\def\bain{Bull~Astron~Inst~Netherlands~} 
                % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund~Cosmic~Phys~}  % Fundamental Cosmic Physics
\def\gca{Geochim~Cosmochim~Acta~}   % Geochimica Cosmochimica Acta
\def\grl{Geophys~Res~Lett~} % Geophysics Research Letters
\def\jcp{J~Chem~Phys~}      % Journal of Chemical Physics
\def\jgr{J~Geophys~Res~}    % Journal of Geophysics Research
\def\jqsrt{J~Quant~Spec~Radiat~Transf~}
                % Journal of Quantitiative Spectroscopy and Radiative Transfer
\def\memsai{Mem~Soc~Astron~Italiana~}
                % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl~Phys~A~}   % Nuclear Physics A
\def\physrep{Phys~Rep~}   % Physics Reports
\def\physscr{Phys~Scr~}   % Physica Scripta
\def\planss{Planet~Space~Sci~}   % Planetary Space Science
\def\procspie{Proc~SPIE~}   % Proceedings of the SPIE

\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

